No-regret learning and mixed Nash equilibria: They do not mix

Understanding the behavior of no-regret dynamics in general $N$-player games is a fundamental question in online learning and game theory. A folk result in the field states that, in finite games, the empirical frequency of play under no-regret learning converges to the game's set of coarse correlated equilibria. By contrast, our understanding of how the day-to-day behavior of the dynamics correlates to the game's Nash equilibria is much more limited, and only partial results are known for certain classes of games (such as zero-sum or congestion games). In this paper, we study the dynamics of "follow-the-regularized-leader" (FTRL), arguably the most well-studied class of no-regret dynamics, and we establish a sweeping negative result showing that the notion of mixed Nash equilibrium is antithetical to no-regret learning. Specifically, we show that any Nash equilibrium which is not strict (in that every player has a unique best response) cannot be stable and attracting under the dynamics of FTRL. This result has significant implications for predicting the outcome of a learning process as it shows unequivocally that only strict (and hence, pure) Nash equilibria can emerge as stable limit points thereof.

==> App-FundDichotomy.tex <==
%----------------------------------------------------------------------
%%% FTRL
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


\begin{comment}
To connect the long-run behavior of \eqref{eq:FTRL} to the \aclp{NE} of the underlying game, we must first understand how the players' mixed strategies evolve under \eqref{eq:FTRL}.
Our goal in this section is to provide some background to this question as a precursor to our analysis in \cref{sec:analysis}.
%In this section, we provide some background to this question, which will form the foundation for our analysis in \cref{sec:analysis}.
To lighten notation, we will drop in what follows the player index $\play$, writing for example $\strat_{\pure}$ instead of the more cumbersome $\strat_{\play\pure_{\play}}$;
we will only reinstate the index $\play$ if absolutely necessary to avoid confusion.


%----------------------------------------------------------------------
%%% SCORES VS. STRATEGIES
%----------------------------------------------------------------------
\para{Scores \vs strategies}

To begin, we note that \eqref{eq:FTRL} exhibits a peculiar duality:
on the one hand, the variables of interest are the players' mixed strategies $\orbit{\run}\in\strats$;
on the other, the dynamics \eqref{eq:FTRL} evolve in the space $\scores$ of the players' score variables $\dorbit{\run}$.
Mixed strategies are determined by the corresponding scores via the players' choice maps $\score \mapsto \strat = \mirror(\score)$, but this is not a two-way street:
as we explain below, the map $\mirror\from\scores\to\strats$ is \emph{not invertible}, so obtaining an autonomous dynamical system on the strategy space $\strats$ is a delicate affair.
 
A first instance of this discrepancy
%between the (primal) strategy space $\strats$ and the (dual) score space $\scores$
arises when considering which strategies are valid outputs of the players' choice map $\mirror$;
formally, \emph{what is the image of the choice maps $\mirror \from \scores \to \strats$?}
\cref{ex:hreg-Eucl,ex:hreg-logit} provide the two archetypal answers to this question:
\PM{Manoli, I leave it up to you if you want to put a figure for this (here or in the supplement).}
\begin{enumerate}

\item
In the entropic case (\cref{ex:hreg-logit}),
the logit choice map $\mirror = \logit$ only returns \emph{fully mixed} strategies (since $\exp(\score)>0$).
Referring to the supplement for the details,
\PM{Just a pointer in case you want to say more about this \textendash\ your call \smiley}
we have
\begin{equation}
\label{eq:logit-inv}
\logit^{-1}(\strat)
	=
	\begin{cases*}
		\log\strat
%			+ \pcone(\strat)
%			+ (1,\dotsc,1) \R
			+ \setdef{(t,\dotsc,t)}{t\in\R}
%			+ \vspan(1,\dotsc,1)
			&\quad
			if $\strat \in \intstrats$,
			\\
		\varnothing
			&\quad
%			\text{if $\strat \in \bd(\strats)$}
			otherwise.
	\end{cases*}
\end{equation}
Therefore, $\logit$ is not surjective;
however, up to a multiple of $(1,\dotsc,1)$, it is \emph{injective}.
\item
In the Euclidean framework of \cref{ex:hreg-Eucl},
%$\hreg(\strat) = (1/2) \norm{\strat}_{2}^{2}$,
every strategy can be obtained from $\mirror = \Eucl$ (after all, $\Eucl(\strat) = \strat$ for all $\strat\in\strats$).
However, the inverse image $\Eucl^{-1}(\strat)$ of $\strat\in\strats$ now contains the entire \emph{polar cone} $\pcone(\strat)$ to $\strats$ at $\strat$;
formally, $\Eucl^{-1}(\strat) = \strat + \pcone(\strat)$ where
\begin{align}
\label{eq:polar}
\pcone(\strat)
	&= \setdef
		{\score\in\scores}
		{\braket{\score}{\stratalt - \strat} \leq 0 \text{ for all } \stratalt\in\strats}
	\notag\\
	&= \setdef
		{\score\in\scores}
		{\score_{\pure} = \score_{\purealt}
			\text{ if }
			\pure,\purealt\in\supp(\strat)
			\text{ and }
			\score_{\pure} \leq 0
			\text{ otherwise}}.
\end{align}
%It is therefore not possible to invert the mapping $\score\mapsto\strat$ to obtain a well-posed system on $\strats$.
Thus $\Eucl$ is now surjective, but it fails to be injective, even modulo a subspace of $\scores$.
\end{enumerate}

%\begin{remark*}
%When $\strat$ is interior, the polar cone to $\strats$ at $\strat$ is just $\pcone(\strat) = \setdef{(t,\dotsc,t)}{t\in\R}$.
%\end{remark*}

The key obstacle to mapping the dynamics \eqref{eq:FTRL} to $\strats$ is the lack of injectivity of $\mirror$.
In turn, this allows us to make two key observations:
\begin{enumerate*}
[(\itshape i\hspace*{.5pt})]
\item
%as far as the dynamics \eqref{eq:FTRL} are concerned,
there is an important dichotomy between boundary and interior states;
and
\item
this dichotomy is linked to whether the underlying choice map is surjective or not.
\end{enumerate*}
We elaborate on this below.


%----------------------------------------------------------------------
%%% PRIMAL DYNAMICS
%----------------------------------------------------------------------
\para{The dynamics of mixed strategies under \eqref{eq:FTRL}}
\end{comment}



%\subsection{Important properties and the steep/non-steep dichotomy}
To proceed with our analysis, we will need to specify the precise requirements for the dynamics' regularizer function $\hreg$.
These are as follows:
\begin{enumerate*}
[(\itshape i\hspace*{.5pt})]
\item
$\hreg\in C_{0}(\R_{+}^{\nPures}) \cap C_{2}(\R_{++}^{\nPures})$,
\ie $\hreg$ is continuous on $\R_{+}^{\nPures}$ and two times continuously differentiable on $\R_{++}^{\nPures}$;
\item
$\hreg$ is strongly convex on $\strats$;
%\ie $\Hess(\hreg(\strat)) \mgeq \hstr \eye$ for some $\hstr>0$ and all $\strat\in\intstrats$;
and
\item
the inverse Hessian $\hmat(\strat) = \Hess(\hreg(\strat))^{-1}$ of $\hreg$ admits a Lipschitz extension to all of $\strats$ such that $\tanvec^{\top} \hmat(\strat) \tanvec > 0$ whenever $\supp(\tanvec) \supseteq \supp(\strat)$.
\end{enumerate*}
These conditions are purely technical in nature and %, as we discuss in the supplement,
they are satisfied by all the regularizers used in practice.
\PM{Which examples should we include in the supplement?}
%We then have the following basic result:
%for the dynamics of the players' mixed strategies under \eqref{eq:FTRL}:


\begin{tcolorbox}[enhanced,width=5in, drop fuzzy shadow southwest, 
                    boxrule=0.4pt,sharp corners,colframe=yellow!80!black,colback=yellow!10]


The following is simply an implication of the optimality of $\point$. We focus on the perspective of an arbitrary player, say $\play$, and for ease of notation we write $\mirror$, $\strat$ and $\dpoint$ instead of $\mirror_\play$, $\point_\play$ and $\dpoint_\play$ respectively.
\end{tcolorbox}


\begin{lemma}
\label{lem:KKT}
$\point=\mirror(\dpoint)$ if and only if there exists a $\mu\in \R$ and $v_\pure\in\mathbb{R}_\geq0$, for all $\pure\in \pures$, such that for all $\pure\in \pures$ (i) $\dpoint_\pure=\frac{\partial \hreg}{\partial \point_\pure}+\mu-v_\pure$ and (ii) $\point_\pure v_\pure=0$
\end{lemma}

\begin{proof}
Recall that $\mirror(\dpoint)
	= \argmax_{\point\in\points} \{ \braket{\dpoint}{\point} - \hreg(\point) \}=\argmax\{\sum_{\pure\in\pures}\dpoint_\pure \point_\pure-\hreg(\point)|\sum_{\pure\in\pures}\point_\pure=1 \mbox{ and } \forall \pure \in\pures:\point_\pure\geq 0\}$. 
The result follows by applying the KKT conditions to this optimization problem and note that, since the constraints are affine, the KKT conditions are sufficient for optimality.
Set (i) of constraints are the stationarity constraints, which in our case are $\nabla( \sum_{\pure\in\pures}\dpoint_\pure \point_\pure - \hreg(\point) )=\mu\nabla(\sum_{\pure\in\pures} \point_\pure-1) - \sum_{\pure\in\pures} v_\pure\nabla \point_\pure$ , while set (ii) of constraints are the complementary slackness constraints.
\end{proof}

Note that complementary slackness implies that whenever $v_\pure>0$, $\pure\notin \supp(\point)$. 






\begin{tcolorbox}[enhanced,width=5in, drop fuzzy shadow southwest, 
                    boxrule=0.4pt,sharp corners,colframe=yellow!80!black,colback=yellow!10]
The following lemma shows that if the support of $\point(t)$ is fixed for a time interval, then a dynamical system arises. Additionally, one can derive that the  trajectory of an $\point(\run)$   coincides with the trajectory that $\point(t)$ would have if the game had only  the strategies of that support. 

Again, for ease of notation  we focus on  player $\play$ and  omit $\play$ from the subscripts
\end{tcolorbox}

\begin{comment}
\begin{proposition}
\label{prop:FTRL-strat}
Let $\orbit{\run} = \mirror(\dorbit{\run})$ be a mixed strategy orbit of \eqref{eq:FTRL}, and let $\runs$ be an interval over which $\supp(\orbit{\run})$ is constant.
%and equal to $\supported\subseteq\pures$.
Then, for all $\run\in\runs$, $\orbit{\run}$ satisfies the mixed strategy dynamics:
\begin{equation}
\label{eq:FTRL-strat}
\tag{\ref*{eq:FTRL}-s}
\dot\strat_{\pure}
	= \insum_{\purealt\in\supp(\strat)}
		\bracks*{\hmat_{\pure\purealt}(\strat) - \hmat_{\pure}(\strat) \hmat_{\purealt}(\strat)}\,
		\payv_{\pure}(\strat),
\end{equation}
where $\hmat_{\pure}(\strat) = \bracks*{\sum_{\purealt,\alt\purealt\in\supp(\strat)} \hmat_{\purealt\alt\purealt}(\strat)}^{-1/2} \sum_{\purealt\in\supp(\strat)} \hmat_{\pure\purealt}(\strat)$.
\end{proposition}
\end{comment}

\begin{lemma}\label{lem:restr_dynamics}
Let $\orbit{\run} = \mirror(\dorbit{\run})$ be a mixed strategy orbit of \eqref{eq:FTRL}, and let $\runs$ be an interval over which $\supp(\orbit{\run})=\pures^*$ is constant.
%and equal to $\supported\subseteq\pures$.
Then, for all $\run\in\runs$, $\orbit{\run}$ satisfies the mixed strategy dynamics:
\begin{equation}%\label{eqn:restr_dynamics}
\label{eq:FTRL-strat}\tag{\ref*{eq:FTRL}-s}
    \dot{\point}_\pure=\sum_{\purealt\in\pures^*}\Big[ g^{\pure\purealt}(t)-\frac{1}{G(\point)}g^\pure(x)g^{\purealt}(x)  \Big]u_{\purealt}(x),
\end{equation}
where
$g^{\pure\purealt}(x)$ is the inverse of the restricted Hessian matrix $H_{\pure\purealt}(x)=\frac{\partial^2\hreg}{\partial\point_\pure\partial\point_\purealt}$, for $\pure,\purealt\in\pures^*$,
$g^\pure(x)=\sum_{\purealt\in\pures^*}g^{\pure\purealt}(x)$ and $G(\point)=\sum_{\pure\in\pures^*}g^\pure(\point)=\sum_{\pure,\purealt\in\pures^*}g^{\pure\purealt}(\point)$
\end{lemma}

\begin{proof}
By Lemma \ref{lem:KKT} we have that $$\dpoint_\pure(t)=g_\pure(t)+\mu(t), \,\,\forall t\in I,\forall\pure\in\pures^*$$

Since $\dpoint_\pure$ and $g_\pure$ are both smooth, so is  $\mu(t)$ and thus differentiating with respect to $t$  we get
\begin{align*}
    \dot{\dpoint}_\pure(t)&=\sum_{\purealt\in\pures}\frac{\partial^2\hreg}{\partial\point_{\purealt}\partial\point_\pure} \dot{\point}_{\purealt}(t)+\dot{\mu}(t)\\
    &=\sum_{\purealt\in\pures^*}\frac{\partial^2\hreg}{\partial\point_{\purealt}\partial\point_\pure} \dot{\point}_{\purealt}(t)+\dot{\mu}(t)
\end{align*}
since for all $t\in I$ and $\purealt \in\pures\setminus\pures^*$, $\point_{\purealt}(t)=0$, and thus $\dot{\point}_\pure(t)=0$. Multiplying with the inverse of the Hessian, and omitting $t$ for brevity, we get
\begin{equation}\label{eq:dynamics_boundary_nonsteep}\dot{\point}_\pure=\sum_{\purealt\in\pures}g^{\pure\purealt}\dot{\dpoint}_{\purealt}+g^\pure\dot{\mu}
\end{equation}
By the definition of the dynamics, $\dot{\dpoint}_{\purealt}=\payv_{\purealt}$ and since the support remains constant $\sum_{\pure\in\pures^*}\dot{\point}_\pure=0$. Summing up \Cref{eq:dynamics_boundary_nonsteep} for $\pure\in\pures^*$ we get $$\sum_{\pure,\purealt\in\pures^*}g^{\pure\purealt}\payv_{\purealt}+G\dot{\mu}=0\Leftrightarrow \dot{\mu}=-\frac{\sum_{\purealt\in\pures^*}g^{\purealt}\payv_{\purealt}}{G}$$
Substituting the latter and $\dot{\dpoint}_{\purealt}=\payv_{\purealt}$ to \Cref{eq:dynamics_boundary_nonsteep} we get the result.
\end{proof}







\begin{comment}
\Cref{prop:FTRL-strat} builds on an earlier result by \citet{MS16}, and we prove it in the supplement.
For now, we quickly discuss how it applies to \cref{ex:hreg-Eucl,ex:hreg-logit}:
\begin{enumerate}

\item
For $\hreg(\strat) = \sum_{\pure} \strat_{\pure} \log\strat_{\pure}$, we have $\hmat(\strat) = \diag(\strat_{1},\dotsc,\strat_{\nPures})$ and $\hmat_{\pure}(\strat) = 1$, so we obtain the \acli{RD}
\begin{equation}
\label{eq:RD}
\tag{RD}
\dot\strat_{\pure}
	= \strat_{\pure} \bracks*{\payv_{\pure}(\strat) - \pay(\strat)}.
\end{equation}

\item
For $\hreg(\strat) = 1/2 \norm{\strat}_{2}^{2}$, we have $\hmat(\strat) = \eye$ and $\hmat_{\pure}(\strat) = \abs{\supp(\strat)}^{-1/2}$.
Thus, \eqref{eq:FTRL-strat} yields the \acdef{PD}
\begin{equation}
\label{eq:PD}
\tag{PD}
\dot\strat_{\pure}
	= \payv_{\pure}(\strat) - \abs{\supp(\strat)}^{-1} \insum_{\purealt\in\supp(\strat)} \payv_{\purealt}(\strat)
		\quad
		\text{if $\pure\in\supp(\strat)$}
%	= \begin{cases*}
%		\payv_{\pure}(\strat) - \abs{\supp(\strat)}^{-1} \sum_{\purealt\in\supp(\strat)} \payv_{\purealt}(\strat)
%			&\quad
%			if $\pure\in\supp(\strat)$,
%		\\
%		0
%			&\quad
%			otherwise.
%	\end{cases*}
\end{equation}
an expression which is valid over all open intervals $\runs$ for which $\supp(\orbit{\run})$ is constant.
\end{enumerate}

The differences between \eqref{eq:PD}\,/\,\eqref{eq:RD} and their relation to the mother scheme \eqref{eq:FTRL} embody the dichotomy to which we alluded before:
\begin{enumerate}
\item
The replicator equation \eqref{eq:RD} is a well-posed dynamical system on all of $\strats$.%
\footnote{Well-posed means here that, for every inital condition, \eqref{eq:RD} admits a unique solution defined over all $\run\geq0$.}
The solutions of \eqref{eq:RD} agree with the mixed strategy orbits $\orbit{\run} = \logit(\dorbit{\run})$ of \eqref{eq:EW} on the interior $\intstrats$ of $\strats$, and they provide a continuous extension thereof to the boundary $\bd(\strats)$ of $\strats$.
\item
The projection dynamics \eqref{eq:PD} do not form an autonomous system on $\strats$;
the mixed strategy orbits $\orbit{\run} = \Eucl(\dorbit{\run})$ of \eqref{eq:ERD} satisfy \eqref{eq:PD} only when they do not transit from one face of $\strats$ to another.
\end{enumerate}

As we show in the supplement, this behavior is intimately tied to the behavior of the derivatives of $\hreg$ at the boundary of $\strats$.
To formalize this, we say that $\hreg$ is \emph{steep} if $\norm{\nabla\hreg(\strat)} \to \infty$ whenever $\strat\to\bd(\strats)$ and $\rank(\hmat(\point)) = \abs{\supp(\point)}$ for all $\strat$;
by contrast, if $\sup_{\strat\in\strats} \norm{\nabla\hreg(\strat)} < \infty$
and $\rank(\hmat(\point)) = \nPures$,
we say that $\hreg$ is \emph{non-steep}.
\PM{\textbf{@all:}
if you prefer different names for steep/non-steep (I recall Manolis wasn't a fan), feel free to suggest alternatives, I'll live \smiley}
Thus, in terms of our examples, the negentropy function of \cref{ex:hreg-logit} is the archetype for steep regularizers, while the $L^{2}$ penalty of \cref{ex:hreg-Eucl} is the non-steep one.
\end{comment}


\begin{tcolorbox}[enhanced,width=5in, drop fuzzy shadow southwest, 
                    boxrule=0.4pt,sharp corners,colframe=yellow!80!black,colback=yellow!10]
The next result unravels the polar split between steep and non-steep dynamics.
\end{tcolorbox}



%With this in mind, our 

\begin{proposition}
\label{prop:dichotomy}
%Let $\hreg$ be a regularizer on $\strats$ and
%Let $\orbit{\run} = \mirror(\dorbit{\run})$ be a mixed strategy orbit of \eqref{eq:FTRL}.
Let $\hreg$ be a regularizer on $\strats$ with induced choice map $\mirror\from\scores\to\strats$.
Then:
%\vspace{\smallskipamount}
\begin{enumerate}
\item
If $\hreg$ is steep:
\begin{enumerate*}
[(\itshape a\upshape)]
\item
$\mirror$ only outputs interior strategies;
\item
\eqref{eq:FTRL-strat} is well-posed on $\strats$
and
$\orbit{\run} = \mirror(\dorbit{\run})$ is a global interior solution thereof.
\end{enumerate*}
%satisfies \eqref{eq:FTRL-strat} for all $\run\geq0$.
\item
If $\hreg$ is non-steep:
\begin{enumerate*}
[(\itshape a\upshape)]
\item
$\mirror$ is surjective;
\item
\eqref{eq:FTRL-strat} is not well-posed
but
$\orbit{\run} = \mirror(\dorbit{\run})$ satisfies \eqref{eq:FTRL-strat} on an open dense set of times \textendash\ to wit, except when $\orbit{\run}$ changes support.
\end{enumerate*}
\end{enumerate}
\end{proposition}

\begin{proof}

\end{proof}


%This separation of regimes \textendash\ steep \vs non-steep \textendash\ underlies much of the analysis to come in an essential way.To streamline our presentation, we defer the proof of \cref{prop:dichotomy} to the supplement.

==> App-Reguralizers.tex <==
%----------------------------------------------------------------------
%%% APP: MIRROR
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is a sample appendix.
It also contains a test equation:
\begin{equation}
\mirror(\dpoint)
	= \argmax_{\point\in\points} \{ \braket{\dpoint}{\point} - \hreg(\point) \}
\end{equation}
Notice the different numbering scheme in the appendix.

==> Figures/main-figures.tex <==
%\input{steepVSnon-steep}
%\input{Grid}\\
%\input{BallFlowSteep}\\
%\input{BallFlowNonSteep}\\
%\input{others}
\input{NewGrid}\\
\input{BallFlow}\\
\input{XYZ}


==> Related.tex <==
%----------------------------------------------------------------------
%%% RELATED
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


\para{Related work}
This is a test citation of \citet{San10} and another for \citet{Wei95}.
This is some more related work, with a test citation of \citet{HS03}.
\PM{Out of curiosity, why a separate section for the related work?
This is not very common for NeurIPS I'd say\dots}

==> Tables/Analysis.tex <==
%----------------------------------------------------------------------
%%% ANALYSIS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


We now turn to the equilibrium convergence properties of \eqref{eq:FTRL}.
The central question that we seek to address here is the following:
\emph{Which \aclp{NE} can be stable and attracting under \eqref{eq:FTRL}?}
\emph{Are all equilibria created equal in that regard?}
%----------------------------------------------------------------------
%%% STABILITY
%----------------------------------------------------------------------
\subsection{Notions of stability}
%To answer this question, we first need to define what ``stable'' and ``attracting'' mean.
At a high level, a point is
\begin{enumerate*}
[(\itshape a\upshape)]
\item
\emph{stable} when every trajectory that starts nearby remains nearby;
and
\item
\emph{attracting} when it attracts all trajectories that start close enough.
\end{enumerate*}
Already, this heuristic shows that defining these notions for \eqref{eq:FTRL} is not straightforward:
the target points are strategy profiles in $\strats$, while the dynamics \eqref{eq:FTRL} evolve in the dual space $\scores$.
When $\hreg$ is \emph{steep},
%based on \cref{sec:FTRL}
we can define an equivalent presentation of \eqref{eq:FTRL} on $\strats$, so this problem can be circumvented by working solely with mixed strategies;
however, when $\hreg$ is \emph{non-steep}, this is no longer possible and we need to navigate carefully between $\strats$ and $\scores$.
In view of this, we have the following definitions:
%\vspace{-\smallskipamount}
\begin{itemize}
\item
$\eq\in\strats$ is \emph{stable} if, for every neighborhood $\nhd$ of $\eq$ in $\strats$, there exists a neighborhood $\alt\nhd$ of $\eq$ such that $\orbit{\run} = \mirror(\dorbit{\run}) \in \nhdalt$ for all $\run\geq0$ whenever $\orbit{\start} = \mirror(\dorbit{\start}) \in \nhdalt$.
\item
$\eq\in\strats$ is \emph{attracting} if there exists a neighborhood $\nhd$ of $\eq$ in $\strats$ such that $\orbit{\run} = \mirror(\dorbit{\run}) \to \eq$ whenever $\orbit{\start} = \mirror(\dorbit{\start}) \in \nhd$.
\item
$\eq\in\strats$ is \emph{asymptotically stable} if it is both stable and attracting.
\end{itemize}
%\vspace{-\smallskipamount}
For obvious reasons, asymptotic stability is the ``gold standard'' for questions pertaining to equilibrium convergence and it will be our litmus test for the appropriateness of an equilibrium $\eq\in\strats$ as an outcome of play.
Specifically, if a \acl{NE} is not asymptotically stable under \eqref{eq:FTRL}, it is not reasonable to expect a no-regret learner to converge to it, meaning in turn that it cannot be justified as an end-state of the players' learning process.
We expound on this below.


%----------------------------------------------------------------------
%%% INCOMPRESSIBILITY
%----------------------------------------------------------------------
\subsection{Volume preservation}

A key observation regarding asymptotic stability is that neighborhoods of initial conditions near an asymptotically stable point should ``contract'' over time, eventually shrinking down to the point in question.
Our first result below provides an apparent contradiction to this principle:
it shows that volume is preserved under \eqref{eq:FTRL},
\emph{irrespective of the underlying game.}

\begin{restatable}
{proposition}{volumeY}
\label{prop:volume}
Let $\region_{\start} \subseteq \scores$ be a set of initial conditions for \eqref{eq:FTRL} and let $\region_{\run} = \setdef{\dorbit{\run}}{\dorbit{\start} \in \region_{\start}}$ denote its evolution under \eqref{eq:FTRL} after time $\run\geq\start$.
Then, $\vol(\region_{\run}) = \vol(\region_{\start})$.
\end{restatable}

\Cref{prop:volume} (which we prove in the supplement through an application of Liouville's formula) is surprising in its universality as it holds for \emph{all games} and \emph{all instances} of \eqref{eq:FTRL}.
As such, it provides a blanket generalization of the well-known volume-preserving property for the replicator dynamics established by \citet{Aki80},
\revise{as well as subsequent results} for zero-sum games \citep{MPP18}.


%----------------------------------------------------------------------
%% Figure for steep/non-steep grid begins here

\begin{figure}[t]
%\vspace{1ex}
\centering
\input{Figures/Grid.tex}
%\includegraphics{Figures/Grid-standalone.pdf}
\caption{The duality between scores and strategies under \eqref{eq:FTRL}:
the dynamics are volume-preserving in $\scores$, but a volume of initial conditions could either collapse in finite time (in the Euclidean case, left), or shrink asymptotically (in the logit case, right).
This is due to the vastly different geometric properties of each system.}
\label{fig:grid}
\end{figure}

%% Figure for steep/non-steep grid ends here
%----------------------------------------------------------------------


%----------------------------------------------------------------------
%%% INTERIOR INSTABILITY
%----------------------------------------------------------------------
\subsection{Instability of fully mixed equilibria}

As stated above, the volume-preserving property of \eqref{eq:FTRL} would seem to suggest that no strategy can be asymptotically stable.
However, this is a figment of the duality between strategy and score variables:
a mixed strategy orbit $\orbit{\run} = \mirror(\dorbit{\run})$ could converge in $\strats$, even though the corresponding dual orbit $\dorbit{\run}$ diverges in $\scores$ (for an illustration, see \cref{fig:grid} above).
This again brings into sharp contrast the behavior of \eqref{eq:FTRL} at the boundary of $\strats$ versus its behavior at the interior.
Our first instability result below shows that the volume-preserving property of \eqref{eq:FTRL} rules out the stability of \emph{any} fully mixed equilibrium, in \emph{any} game:

\begin{restatable}{theorem}{stableInt}
\label{thm:unstable-int}
A fully mixed \acl{NE} cannot be asymptotically stable under \eqref{eq:FTRL}.
\end{restatable}

The main idea of the proof of \cref{thm:unstable-int} relies on a tandem application of \cref{prop:volume} together with the dimensionality reduction idea we discussed for the entropic case in \cref{sec:FTRL}.
In the resulting quotient space, the inverse image of an interior point $\eq\in\intstrats$ is a single point and the induced dynamics remain volume-preserving.
If $\eq$ is asymptotically stable, a limit point argument rules out the possibility of a trajectory entering and exiting a small neighborhood of its preimage infinitely many times.
At the same time, Lyapunov stability and volume preservation imply that the dynamics are locally recurrent.
This contradicts the transient property established above and proves that $\eq$ cannot be asymptotically stable;
the details involved in making these arguments precise are fairly intricate, so we defer the proof of \cref{thm:unstable-int} to the supplement.

%From an epistemic viewpoint,
This universal instability result has significant implications as it provides a dynamic justification of the fragility of fully mixed \aclp{NE}.
%Indeed, if a single player makes a small mistake in implementing a fully mixed strategy, all players could be thrown out of equilibrium because of this error \citep{FT91,LRS19}.
\Cref{thm:unstable-int} illustrates this principle through the lens of regret minimization:
any deviation from a fully mixed equilibrium invariably creates an opportunity that can be exploited by a no-regret learner.
When every player adheres to such a policy, this creates a vicious cycle which destroys any chance of stability for fully mixed equlibria.


%----------------------------------------------------------------------
%%% MIXED INSTABILITY
%----------------------------------------------------------------------
\subsection{The case of partially mixed equilibria}
Taking this premise to its logical extreme, a natural question that arises is whether this instability persists as long as even a \emph{single} player employs a mixed strategy at equilibrium. In the previous case, after the dimensionality reduction argument we described in \cref{sec:FTRL}, \revise{neighborhoods of} fully mixed equilibria \revise{in the space of strategies ($\strats$) correspond to sets of finite volume in the space of payoffs ($\scores$).}
On the contrary, the case of \emph{partially} mixed equilibria is much more complex
%since they would be mapped to a set of infinite volume using the polar cone arguments
\revise{because neighborhoods of points on the boundary of $\strats$ correspond to sets of \emph{infinite} volume in the space of payoffs} 
\textendash\ and this, even after dimensionality reduction (\cf \cref{fig:polarcone}).
Because of this, volume preservation arguments cannot rule out asymptotic stability of \revise{\aclp{NE} lying at the boundary of the strategy space:}
indeed, pure \aclp{NE} also lie on the boundary but they \emph{can} be asymptotically stable \citep{MS16}.
%consequently, a more precise argument is needed for the intermediate case of partially mixed equilibria.

\revise{In view of the above, it is not a priori clear whether partially mixed equilibria would behave more like pure or fully mixed ones \textendash\ or if no conclusion can be drawn whatsoever.
Our next result shows that the dynamics of \ac{FTRL} represent a very sharp selection mechanism in this regard:}


%\begin{comment}
%Taking this premise to its logical extreme, a natural question that arises is whether this instability persists as long as even a \emph{single} player employs a mixed strategy at equilibrium.
%Indeed, if an agent has several best responses at equilibrium, any switch to an alternative best-response would not incur any regret on the deviating player, but it could potentially trigger a vicious cycle of changes by the other no-regret learners (who might be presented with an opportunity to exploit).
%%Since each player's best-response correspondence is upper hemicontinuous, a deviation by the mixing player could potentially trigger a similar vicious cycle between no-regret learners,
%%suggesting a positive answer to the above question.
%%implying in turn that mixed equilibria cannot be stable under \eqref{eq:FTRL}.
%Our next result provides a definitive confirmation of this hypothesis:
%\end{comment}

\begin{restatable}{theorem}{stableMixed}
\label{thm:unstable-mixed}
Only strict \aclp{NE} can be asymptotically stable under \eqref{eq:FTRL}.
\end{restatable}



\begin{corollary}
\label{cor:stable-strict}
If $\eq$ is partially mixed, it cannot be asymptotically stable under \eqref{eq:FTRL}.
\end{corollary}

Viewed in isolation, \cref{thm:unstable-int} would seem to be subsumed by \cref{thm:unstable-mixed}, but this is not so:
the former plays an integral role in the proof of the latter, so it cannot be viewed as a special case.
In more detail, the proof of \cref{thm:unstable-mixed} builds on \cref{thm:unstable-int} along two separate axes, depending on whether the underlying regularizer is steep or not:

\begin{enumerate}
[leftmargin=*]
\item
In the steep case, as we discussed in \cref{sec:FTRL} there is a well-posed dynamical system on $\strats$.
As we show in the supplement, each face of $\strats$ is forward-invariant in this system,
so $\eq$ must also be asymptotically stable when constrained to the face of $\eqs$ of $\strats$ spanned by $\supp(\eq)$.
The conclusion of \cref{thm:unstable-mixed} then follows by noting that $\eq$ is interior in $\eqs$ and applying \cref{thm:unstable-int} to the restriction of the underlying game to $\eqs$.
%\vspace{-0.2cm}
\item
The non-steep case is considerably more difficult because \eqref{eq:FTRL} no longer induces a well-posed system on $\strats$.
In lieu of this, by examining the finer structure of the inverse image of $\eq$, it is possible to show the following:
for every small enough compact neighborhood $\cpt$ of $\eq$ in $\strats$, there exists a finite time $\tau_{\cpt} \geq 0$ such that $\supp(\orbit{\run}) = \supp(\eq)$ for all $\run\geq\tau_{\cpt}$ whenever $\orbit{\start} \in \cpt$.
As it turns out, the dynamics after $\run\geq\tau_{\cpt}$ \revise{loca}lly coincide with the mixed strategy dynamics of \eqref{eq:FTRL} applied to the restriction of the underlying game to the face $\eqs$ of $\strats$ spanned by $\eq$.
Since $\eq$ is a fully mixed equilibrium in this restricted game, it cannot be asymptotically stable.
\end{enumerate}

%----------------------------------------------------------------------
%%% SETWISE STABILITY
%----------------------------------------------------------------------
\subsection{Stable limit sets}

We conclude our analysis with a result concerning more general behaviors whereby the dynamics of \ac{FTRL} do not converge to a point, but to a more general \emph{invariant set} \textendash\ such as a chain of stationary points interconnected by solution orbits, a structure known as a \emph{heteroclinic cycle} \citep[see \eg][and references therein]{HS98,San10}. % and references therein.
As an example, in the case of two-player zero-sum games with a fully mixed equilibrium, it is known that the trajectories of \eqref{eq:FTRL} form periodic orbits (cycles).
However, these orbits are \emph{not} asymptotically stable:
if the initialization of the \ac{FTRL} dynamics is slightly perturbed, the resulting trajectory will be a different periodic orbit, which does not converge to the first (in the language of dynamical systems, the cycles observed in zero-sum games are not \emph{limit cycles}).
We are thus led to the following natural question:
%\vspace{-\smallskipamount}
\begin{center}
\emph{What type of invariant structures can arise as stable limits of \eqref{eq:FTRL}?}
\end{center}
%\vspace{-\smallskipamount}
To state this question formally, we will require the setwise version of asymptotic stability:
a set $\set$ is called \emph{asymptotically stable} under \eqref{eq:FTRL} if
\begin{enumerate*}
[\itshape a\upshape)]
%\addtolength{\itemsep}{-\smallskipamount}
\item
all orbits $\orbit{\run} = \mirror(\dorbit{\run})$ of \eqref{eq:FTRL} that start sufficiently close to $\set$ remain close;
and
\item
all orbits that start nearby eventually converge to $\set$.
\end{enumerate*}
Then, focusing on the case of steep dynamics to avoid more complicated statements, we have:

\begin{restatable}{theorem}{stableSet}
\label{thm:unstable-set}
Every asymptotically stable set of steep \eqref{eq:FTRL} contains a pure strategy.
%Suppose that $\set$ is asymptotically stable under \eqref{eq:FTRL} with a steep regularizer.
%Then $\set$ contains a pure strategy profile $\eq[\pure] \in \pures$.
\end{restatable}

The proof of \cref{thm:unstable-set} relies on an ``infinite descent'' argument whereby the faces of $\points$ that intersect with $\set$ are eliminated one-by-one, until only pure strategies remain as candidate elements of $\set$ with minimal support;
we provide the details in the supplement.

The importance of \cref{thm:unstable-set}
%Its importance
lies in that it provides a succinct criterion for identifying possible attracting sets of \eqref{eq:FTRL}.
Indeed, by Conley's decomposition theorem (also known as the ``fundamental theorem of dynamical systems'') \citep{Con78}, the flow of \eqref{eq:FTRL} in an arbitrary game decomposes into a chain recurrent part and an attracting part.
The recurrent part is exemplified by the periodic orbits that arise in zero-sum games with an interior equilibrium (there are no attractors in this case) \citep{MPP18}.
\Cref{thm:unstable-set} goes a long way to showing that the attracting part of \eqref{eq:FTRL} always intersects the \emph{extremes} of the game's strategy space \textendash\ \ie the players' set of \emph{pure} strategies.
Formalizing the exact form of this decomposition in arbitrary games is an open direction for future reserach with far-reaching implications for the theory of online learning in games.
